Adaptively Weighted Data Augmentation Consistency Regularization for Robust Optimization under Concept Shift

Concept shift is a prevailing problem in natural tasks like medical image segmentation where samples usually come from different subpopulations with variant correlations between features and labels. One common type of concept shift in medical image segmentation is the "information imbalance" between label-sparse samples with few (if any) segmentation labels and label-dense samples with plentiful labeled pixels. Existing distributionally robust algorithms have focused on adaptively truncating/down-weighting the "less informative" (i.e., label-sparse in our context) samples. To exploit data features of label-sparse samples more efficiently, we propose an adaptively weighted online optimization algorithm -- AdaWAC -- to incorporate data augmentation consistency regularization in sample reweighting. Our method introduces a set of trainable weights to balance the supervised loss and unsupervised consistency regularization of each sample separately. At the saddle point of the underlying objective, the weights assign label-dense samples to the supervised loss and label-sparse samples to the unsupervised consistency regularization. We provide a convergence guarantee by recasting the optimization as online mirror descent on a saddle point problem. Our empirical results demonstrate that AdaWAC not only enhances the segmentation performance and sample efficiency but also improves the robustness to concept shift on various medical image segmentation tasks with different UNet-style backbones.

==> format.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
% \RequirePackage{hyperref}
\RequirePackage{enumitem}

% %%%%%%%%%%%%%%% hyperref %%%%%%%%%%%%%%%
% \definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \hypersetup{
%     pdftoolbar=true,        % show Acrobat’s toolbar?
%     pdfmenubar=true,        % show Acrobat’s menu?
%     pdffitwindow=false,     % window fit to page when opened
%     pdfstartview={FitH},    % fits the width of the page to the window
%     pdftitle={title},    % title
%     pdfnewwindow=true,      % links in new window
%     colorlinks=true,
%     linkcolor=mydarkblue,
%     citecolor=mydarkblue,
%     filecolor=mydarkblue,
%     urlcolor=mydarkblue,
% }



%%%%%%%%%%%%%%% theorems %%%%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
    \theoremstyle{definition}
\newtheorem{definition}{Definition}
    \theoremstyle{definition}
\newtheorem{assumption}{Assumption}
    \theoremstyle{remark}
\newtheorem{remark}{Remark}
    \theoremstyle{remark}
\newtheorem{conjecture}{Conjecture}
    \theoremstyle{definition}
\newtheorem{example}{Example}
\numberwithin{equation}{section}
\numberwithin{figure}{section}



%%%%%%%%%%%%%%% Special characters %%%%%%%%%%%%%%%
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}} % complex field
\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}} % nature numbers
\newcommand{\OO}{\mathbb{O}} % nature numbers
\newcommand{\PP}{\mathbb{P}} % nature numbers
\newcommand{\Q}{\mathbb{Q}} % rational field 
\newcommand{\R}{\mathbb{R}} % real field
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}} % integer field



% bold
\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\renewcommand{\sb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}


\newcommand{\abd}{\boldsymbol{a}}
\newcommand{\bbd}{\boldsymbol{b}}
\newcommand{\cbd}{\boldsymbol{c}}
\newcommand{\dbd}{\boldsymbol{d}}
\newcommand{\ebd}{\boldsymbol{e}}
\newcommand{\fbd}{\boldsymbol{f}}
\newcommand{\gbd}{\boldsymbol{g}}
\newcommand{\hbd}{\boldsymbol{h}}
\newcommand{\ibd}{\boldsymbol{i}}
\newcommand{\jbd}{\boldsymbol{j}}
\newcommand{\kbd}{\boldsymbol{k}}
\newcommand{\lbd}{\boldsymbol{l}}
\newcommand{\mbd}{\boldsymbol{m}}
\newcommand{\nbd}{\boldsymbol{n}}
\newcommand{\obd}{\boldsymbol{o}}
\newcommand{\pbd}{\boldsymbol{p}}
\newcommand{\qbd}{\boldsymbol{q}}
\newcommand{\rbd}{\boldsymbol{r}}
\newcommand{\sbd}{\boldsymbol{s}}
\newcommand{\tbd}{\boldsymbol{t}}
\newcommand{\ubd}{\boldsymbol{u}}
\newcommand{\vbd}{\boldsymbol{v}}
\newcommand{\wbd}{\boldsymbol{w}}
\newcommand{\xbd}{\boldsymbol{x}}
\newcommand{\ybd}{\boldsymbol{y}}
\newcommand{\zbd}{\boldsymbol{z}}

\newcommand{\Abd}{\boldsymbol{A}}
\newcommand{\Bbd}{\boldsymbol{B}}
\newcommand{\Cbd}{\boldsymbol{C}}
\newcommand{\Dbd}{\boldsymbol{D}}
\newcommand{\Ebd}{\boldsymbol{E}}
\newcommand{\Fbd}{\boldsymbol{F}}
\newcommand{\Gbd}{\boldsymbol{G}}
\newcommand{\Hbd}{\boldsymbol{H}}
\newcommand{\Ibd}{\boldsymbol{I}}
\newcommand{\Jbd}{\boldsymbol{J}}
\newcommand{\Kbd}{\boldsymbol{K}}
\newcommand{\Lbd}{\boldsymbol{L}}
\newcommand{\Mbd}{\boldsymbol{M}}
\newcommand{\Nbd}{\boldsymbol{N}}
\newcommand{\Obd}{\boldsymbol{O}}
\newcommand{\Pbd}{\boldsymbol{P}}
\newcommand{\Qbd}{\boldsymbol{Q}}
\newcommand{\Rbd}{\boldsymbol{R}}
\newcommand{\Sbd}{\boldsymbol{S}}
\newcommand{\Tbd}{\boldsymbol{T}}
\newcommand{\Ubd}{\boldsymbol{U}}
\newcommand{\Vbd}{\boldsymbol{V}}
\newcommand{\Wbd}{\boldsymbol{W}}
\newcommand{\Xbd}{\boldsymbol{X}}
\newcommand{\Ybd}{\boldsymbol{Y}}
\newcommand{\Zbd}{\boldsymbol{Z}}


\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}



\newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\Bfrak}{\mathfrak{B}}
\newcommand{\Cfrak}{\mathfrak{C}}
\newcommand{\Dfrak}{\mathfrak{D}}
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\Ffrak}{\mathfrak{F}}
\newcommand{\Gfrak}{\mathfrak{G}}
\newcommand{\Hfrak}{\mathfrak{H}}
\newcommand{\Ifrak}{\mathfrak{I}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\Kfrak}{\mathfrak{K}}
\newcommand{\Lfrak}{\mathfrak{L}}
\newcommand{\Mfrak}{\mathfrak{M}}
\newcommand{\Nfrak}{\mathfrak{N}}
\newcommand{\Ofrak}{\mathfrak{O}}
\newcommand{\Pfrak}{\mathfrak{P}}
\newcommand{\Qfrak}{\mathfrak{Q}}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Sfrak}{\mathfrak{S}}
\newcommand{\Tfrak}{\mathfrak{T}}
\newcommand{\Ufrak}{\mathfrak{U}}
\newcommand{\Vfrak}{\mathfrak{V}}
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\Xfrak}{\mathfrak{X}}
\newcommand{\Yfrak}{\mathfrak{Y}}
\newcommand{\Zfrak}{\mathfrak{Z}}


% Greek
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\epsb}{\boldsymbol{\eps}}
\newcommand{\vepsb}{\boldsymbol{\veps}}
\newcommand{\zetab}{\boldsymbol{\zeta}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\vthetab}{\boldsymbol{\vartheta}}
\newcommand{\iotab}{\boldsymbol{\iota}}
\newcommand{\kappab}{\boldsymbol{\kappa}}
\newcommand{\vkappab}{\boldsymbol{\varkappa}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\omicronb}{\boldsymbol{\omicron}}
\newcommand{\pib}{\boldsymbol{\pi}}
\newcommand{\vpib}{\boldsymbol{\varpi}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\vrhob}{\boldsymbol{\varrho}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\vsigmab}{\boldsymbol{\varsigma}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\upsilonb}{\boldsymbol{\upsilon}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\vphib}{\boldsymbol{\varphi}}
\newcommand{\chib}{\boldsymbol{\chi}}
\newcommand{\psib}{\boldsymbol{\psi}}
\newcommand{\omegab}{\boldsymbol{\omega}}

\newcommand{\Alphab}{\boldsymbol{\Alpha}}
\newcommand{\Betab}{\boldsymbol{\Beta}}
\newcommand{\Gammab}{\boldsymbol{\Gamma}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Epsb}{\boldsymbol{\Epsilon}}
\newcommand{\Zetab}{\boldsymbol{\Zeta}}
\newcommand{\Etab}{\boldsymbol{\Eta}}
\newcommand{\Thetab}{\boldsymbol{\Theta}}
\newcommand{\Iotab}{\boldsymbol{\Iota}}
\newcommand{\Kappab}{\boldsymbol{\Kappa}}
\newcommand{\Lambdab}{\boldsymbol{\Lambda}}
\newcommand{\Mub}{\boldsymbol{\Mu}}
\newcommand{\Nub}{\boldsymbol{\Nu}}
\newcommand{\Xib}{\boldsymbol{\Xi}}
\newcommand{\Omicronb}{\boldsymbol{\Omicron}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\Rhob}{\boldsymbol{\Rho}}
\newcommand{\Sigmab}{\boldsymbol{\Sigma}}
\newcommand{\Taub}{\boldsymbol{\Tau}}
\newcommand{\Upsilonb}{\boldsymbol{\Upsilon}}
\newcommand{\Phib}{\boldsymbol{\Phi}}
\newcommand{\Chib}{\boldsymbol{\Chi}}
\newcommand{\Psib}{\boldsymbol{\Psi}}
\newcommand{\Omegab}{\boldsymbol{\Omega}}








%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand{\dfeq}{\triangleq}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\pinv}{\dagger}
\newcommand*{\poly}{\mathop{\mathrm{poly}}}
\newcommand*{\mean}{\mathop{\mathrm{mean}}}
\newcommand*{\median}{\mathop{\mathrm{median}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\prox}{\mathop{\mathrm{prox}}}
\newcommand{\proj}{\mathop{\mathrm{proj}}}
\newcommand{\spn}{\mathop{\mathrm{span}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
\newcommand{\nucnorm}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
\newcommand{\pto}{\mathrel{\ooalign{\hfil$\mapstochar\mkern5mu$\hfil\cr$\to$\cr}}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{\partial #1^2}}
\newcommand{\pnwrt}[2]{\frac{\partial^#1}{\partial #2^#1}}
\newcommand{\pfrac}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppfrac}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pnfrac}[3]{\frac{\partial^#1 #2}{\partial #3^#1}}

\newcommand{\eproof}{$\null\hfill\blacksquare$}
% \renewcommand\qedsymbol{$\blacksquare$}



%%%%%%%%%%%%%%% Super/sup-scripts %%%%%%%%%%%%%%%
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\ol}[1]{\overline{#1}} % overline
\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}




%%%%%%%%%%%%%%% Short Forms %%%%%%%%%%%%%%%
\newcommand{\ea}{\emph{et al.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\iid}{\emph{i.i.d.}\xspace}
\newcommand{\cf}{\emph{cf.}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\st}{\emph{s.t.}\xspace}
\newcommand{\whp}{\emph{w.h.p.}\xspace}



%%%%%%%%%%%%%%% Brackets %%%%%%%%%%%%%%
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abbr}[1]{\left|#1\right|}
\newcommand{\abr}[1]{\langle#1\rangle}
\newcommand{\nnbr}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

\newcommand{\rsep}[2]{\left(#1 \middle| #2 \right)}
\newcommand{\ssep}[2]{\left[#1 \middle| #2 \right]}
\newcommand{\csep}[2]{\left\{#1 \middle| #2 \right\}}
\newcommand{\asep}[2]{\langle#1 \mid #2 \rangle}
\newcommand{\rsepp}[2]{\left(#1 ~\middle|~ #2 \right)}
\newcommand{\ssepp}[2]{\left[#1 ~\middle|~ #2 \right]}
\newcommand{\csepp}[2]{\left\{#1 ~\middle|~ #2 \right\}}
\newcommand{\asepp}[2]{\langle#1 ~\mid~ #2 \rangle}

\newcommand{\apar}[1]{\langle #1 \rangle}
\newcommand{\cpar}[1]{\{#1\}}
\newcommand{\bpar}[1]{\Big( #1 \Big)}
\newcommand{\Bpar}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bspar}[1]{\Big[ #1 \Big]}
\newcommand{\Bspar}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bcpar}[1]{\Big\{ #1 \Big\}}
\newcommand{\Bcpar}[1]{\Bigg\{ #1 \Bigg\}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inpr}[2]{\langle #1, #2 \rangle}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}




%%%%%%%%%%%%%%% Miscellaneous %%%%%%%%%%%%%%%
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\renewcommand{\b}{\textbf}
\renewcommand{\t}[1]{\text{#1}}
% starred section table of contents
\newcommand{\sectiontoc}[1]{
\section*{#1}
\addcontentsline{toc}{section}{\protect\numberline{}#1}%
}


% Local
\newcommand{\yijun}[1]{\blue{[yijun: #1]}}
\newcommand{\needref}{\textcolor{red}{\textbf{@@ref}}}
\newcommand{\dl}{\textit{DL}}
\newcommand{\dsc}{\textit{DSC}}
\newcommand{\iloc}[2]{{#1}_{[#2]}}
\newcommand{\iffun}[1]{\II\cbr{#1}}
\newcommand{\erm}{\textit{ERM}}
\newcommand{\dac}{\textit{AC}}
\newcommand{\wdac}{\textit{WAC}}
\newcommand{\dice}{\textit{DICE}}
\newcommand{\ce}{\textit{CE}}
\newcommand{\Fnb}[1]{\Fcal_{\theta^*}\rbr{#1}}
\newcommand{\lambdac}{\lambda_{\textit{AC}}}
\newcommand{\lossce}{\ell_{\textit{CE}}}
\newcommand{\lossdice}{\ell_{\textit{DICE}}}
\newcommand{\regdac}{\ell_{\textit{AC}}}
\newcommand{\vspacetable}{\vspace{-1em}}











